Topological field theories on open-closed $r$-spin surfaces

In this article, we establish a connection between two models for $r$-spin structures on surfaces: the marked PLCW decompositions of Novak and Runkel-Szegedy, and the structured graphs of Dyckerhoff-Kapranov. We use these models to describe $r$-spin structures on open-closed bordisms, leading to a generators-and-relations characterization of the 2-dimensional open-closed $r$-spin bordism category. This results in a classification of 2-dimensional open closed field theories in terms of algebraic structures we term "knowledgeable $\Lambda_r$-Frobenius algebras". We additionally extend the state sum construction of closed $r$-spin TFTs from a $\Lambda_r$-Frobenius algebra $A$ with invertible window element of Novak and Runkel-Szegedy to the open-closed case. The corresponding knowledgeable $\Lambda_r$-Frobenius algebra is $A$ together with the $\mathbb{Z}/r$-graded center of $A$.

==> gr-occurs <==
appendix.tex:			\tikzfig{move2b}
combinatorial_models.tex:  \tikzfig{graphics/ccw-vertex}
combinatorial_models.tex:		\tikzfig{fixmoves}
combinatorial_models.tex:		\tikzfig{edgemove}
field_theories.tex:	&\tikzfig{Bord-gen-pants},
field_theories.tex:	&&\tikzfig{Bord-gen-copants},
field_theories.tex:	&&\tikzfig{Bord-gen-cup},
field_theories.tex:	&&\tikzfig{Bord-gen-cap},
field_theories.tex:	&&\tikzfig{Bord-gen-cylinder}\ ,
field_theories.tex:	\tikzfig{Bord-comp-Nx}
field_theories.tex:	&\tikzfig{Bord-gen-o-pants},
field_theories.tex:	&&\tikzfig{Bord-gen-o-copants},
field_theories.tex:	&&\tikzfig{Bord-gen-o-cup},
field_theories.tex:	&&\tikzfig{Bord-gen-o-cap},
field_theories.tex:	&&\tikzfig{Bord-gen-o-cylinder}\ .
field_theories.tex:	\tikzfig{Bord-gen-o-N}\ .
field_theories.tex:	\tikzfig{Bord-gen-zip}\quad\text{and}\quad
field_theories.tex:	\tikzfig{Bord-gen-cozip}.
field_theories.tex:	\tikzfig{Bord-rel-associativity}
field_theories.tex:	\tikzfig{Bord-rel-Frobenius}
field_theories.tex:		\tikzfig{Bord-rel-N-power}\ .
field_theories.tex:		\tikzfig{Bord-rel-commutativity}
field_theories.tex:		\tikzfig{Bord-rel-SL2Z}
field_theories.tex:	\tikzfig{Bord-rel-center}
field_theories.tex:		\tikzfig{Bord-rel-Cardy}
field_theories.tex:		\tikzfig{Bord-rel-duality}
field_theories.tex:		\tikzfig{Bord-rel-pairing}
frobenius_algebras.tex:	\tikzfig{C-morphisms}
frobenius_algebras.tex:	\tikzfig{C-morphisms-Nx}\ .
frobenius_algebras.tex:	\tikzfig{C-morphisms-relations-alg}\ ,
frobenius_algebras.tex:	\tikzfig{C-morphisms-relations-coalg}\ ,
frobenius_algebras.tex:	\tikzfig{C-morphisms-relations-Frobenius}\ ,
frobenius_algebras.tex:  \tikzfig{C-morphism-relations-deck}\ ,
frobenius_algebras.tex:	\tikzfig{C-morphisms-relations-commutativity}\ ,
frobenius_algebras.tex:	\tikzfig{C-morphisms-relations-twist}\ ,
frobenius_algebras.tex:	\tikzfig{C-morphisms-relations-SL2Z}\ .
frobenius_algebras.tex:		\tikzfig{C-duality-morphisms}
frobenius_algebras.tex:		\tikzfig{cat-dim}
frobenius_algebras.tex:		\tikzfig{torus-xy}
frobenius_algebras.tex:	 \tikzfig{A-morphisms}
frobenius_algebras.tex:		&\tikzfig{AC-rel-knowledge}
frobenius_algebras.tex:		&\tikzfig{AC-rel-duality}
frobenius_algebras.tex:		&\tikzfig{AC-rel-Cardy}
frobenius_algebras.tex:	\tikzfig{idempot-Px}
frobenius_algebras.tex:	\tikzfig{graded-center-morphisms}
field_theories.tex:		\includegraphics{./graphics/Bord_loops.pdf}
field_theories.tex:		\includegraphics{graphics/diff_isot_to_id.pdf}

